heSRPT: Optimal Parallel Scheduling of Jobs With Known Sizes

When parallelizing a set of jobs across many servers, one must balance a trade-off between granting priority to short jobs and maintaining the overall efficiency of the system. When the goal is to minimize the mean flow time of a set of jobs, it is usually the case that one wants to complete short jobs before long jobs. However, since jobs usually cannot be parallelized with perfect efficiency, granting strict priority to the short jobs can result in very low system efficiency which in turn hurts the mean flow time across jobs. In this paper, we derive the optimal policy for allocating servers to jobs at every moment in time in order to minimize mean flow time across jobs. We assume that jobs follow a sublinear, concave speedup function, and hence jobs experience diminishing returns from being allocated additional servers. We show that the optimal policy, heSRPT, will complete jobs according to their size order, but maintains overall system efficiency by allocating some servers to each job at every moment in time. We compare heSRPT with state-of-the-art allocation policies from the literature and show that heSRPT outperforms its competitors by at least 30%, and often by much more.

==> arrivals.tex <==
\section{Handling Arrivals Over Time}
add arrivals


==> future.tex <==
\section{To Do}

Here is a list of tasks we'd like to do in order of priority:

\begin{enumerate}

\item Fix the speedup issue when jobs get $<1$ core.  

\item See if the speedup curve can be generalized.   

\item Big project:   Move to 2 speedup functions.  Specifically, assume that there are $L$ jobs with low parallelizability and $H$ jobs with high parallelizability.  The total number of jobs is $M$, where $M = L + H$.    We should be able to argue that among each group, the jobs will complete smallest-first.   Thus in any stage, the next completion will either be the smallest of the low parallelizability jobs or the smallest of the high parallelizability jobs.  As a first step, we need to determine which of these it will be.     Alternatively, we might be able to determine which fraction of the resource should go to the low parallelizability jobs and which fraction to the high parallelizability jobs.  Then, within each group, we might be able to use our existing formula.   

\item A final item is to consider what happens when the job sizes are not known, but the job size distribution is known.  Here we want to use a Gittins Index ranking among the jobs.   We will need to get arrivals working before we start this.   Also, we'll need to prove that Gittins is optimal in this setting ... (Ben, I was thinking about this, and that's not obvious).

\end{enumerate}



